Bitcoin Battle: Burning Bitcoin for Geopolitical Fun and Profit

This study empirically analyzes the transaction activity of Bitcoin addresses linked to Russian intelligence services, which have liquidated over 7 Bitcoin (BTC), i.e., equivalent to approximately US$300,000 based on the exchange rate at the time. Our investigation begins with an observed anomaly in transaction outputs featuring the Bitcoin Script operation code, tied to input addresses identified by cyber threat intelligence sources and court documents as belonging to Russian intelligence agencies. We explore how an unauthorized entity appears to have gained control of the associated private keys, with messages embedded in the outputs confirming the seizure. Tracing the funds' origins, we connect them to cryptocurrency mixers and establish a link to the Russian ransomware group Conti, implicating intelligence service involvement. This analysis represents one of the first empirical studies of large-scale Bitcoin misuse by nation-state cyber actors.

==> chapters/alternative_hypotheses.tex <==
\section{Alternative Hypotheses}
Inside Job: The Bitcoin was taken by someone from within the GRU, FSB and SVR — a disgruntled operator, or an IT employee with access to key internal systems. This could be for financial gain, personal vendettas, or even as part of a larger scheme orchestrated by external actors.

Rogue Insider Collaboration: An employee (or multiple employees) might have collaborated with a third party. The insiders provided crucial access to the company’s systems or their expertise in bypassing security protocols, allowing the external hacker to execute the theft.

Exploitation of a Wallet Vulnerability: The GRU's Bitcoin wallet could have had an  vulnerability —  a flaw in the software or a mistake made in the implementation of cryptographic protocols — that allowed an attacker to access and steal the funds. This could suggest that while the hacking actor was sophisticated, the company itself made a critical oversight.

Man-in-the-Middle Attack: The Bitcoin theft could be the result of a more subtle attack method, such as a man-in-the-middle attack where a hacker intercepts communication between parties, such as during a transaction or wallet transfer process, without the GRU realizing they were being compromised.

Cryptojacking: The Bitcoin stolen could be linked to cryptojacking — a scenario where the GRU’s systems were compromised, and the hacker mined Bitcoin in a background process without the company’s knowledge and exfiltrating them afterwartds.

==> chapters/methodology.tex <==
\subsection{Methodology}
To gather the \opret\ binary metadata central to this analysis, we used a full node running Bitcoin {\tt Core version 26.2}, synchronized with the blockchain until July 2024. To expedite analysis we used the \textit{blockchain-parser} library \cite{blockparser} to convert Bitcoin-native raw blk*****.dat files, based on the \textit{getrawtransaction} RPC command to plain text. The resulting text files were parsed on the fly for transactions containing \opret\ opcodes using regular expressions, the output of which was pushed to a DataFrame object for efficient querying and data manipulation, ran in memory on a workstation with significant (128 GB) RAM.

Upon obtaining the initial set of suspicious transaction hashes, the parsed Bitcoin data was crawled to discover associated inputs, outputs, and additional transactions. Data was obtained from the free Blockchain.com API~\cite{XXX} for a sample of transaction hashes. This allowed the verification of the results from our parser, which served as a double-check. We were provided access, and we used the Graphsense API maintained by Iknaio for its address clustering capabilities, based on the co-spend heuristic~\cite{meiklejohn2013fistful} to discover joint address ownership. We were also provided access to address labels by Scorechain~\cite{XXX} under an academic license to identify links with counterparties.

A full list of the addresses in our dataset and their derived labels (GRU, SVR, FSB) is available online at ... (to be uploaded after acceptance of the paper).

% add more after receiving approval from Chainalysis
%In addition to this, to trace the origins of funds to the addresses in our dataset, Chainalysis was used.
